The Heuristic Core: Understanding Subnetwork Generalization in Pretrained Language Models

Prior work has found that pretrained language models (LMs) fine-tuned with different random seeds can achieve similar in-domain performance but generalize differently on tests of syntactic generalization. In this work, we show that, even within a single model, we can find multiple subnetworks that perform similarly in-domain, but generalize vastly differently. To better understand these phenomena, we investigate if they can be understood in terms of "competing subnetworks": the model initially represents a variety of distinct algorithms, corresponding to different subnetworks, and generalization occurs when it ultimately converges to one. This explanation has been used to account for generalization in simple algorithmic tasks ("grokking"). Instead of finding competing subnetworks, we find that all subnetworks -- whether they generalize or not -- share a set of attention heads, which we refer to as the heuristic core. Further analysis suggests that these attention heads emerge early in training and compute shallow, non-generalizing features. The model learns to generalize by incorporating additional attention heads, which depend on the outputs of the "heuristic" heads to compute higher-level features. Overall, our results offer a more detailed picture of the mechanisms for syntactic generalization in pretrained LMs.

==> sections/analysis.tex <==
\begin{figure*}[t]
\centering
\subfloat[Layer $3$, Head $7$]{
    \includegraphics[width=0.25\linewidth]{figures/a3h7-1.pdf}
}
\subfloat[Layer $4$, Head $0$]{
    \includegraphics[width=0.25\linewidth]{figures/a4h0-1.pdf}
}
\subfloat[Layer $8$, Head $11$]{
    \includegraphics[width=0.25\linewidth]{figures/a8h11-1.pdf}
}
\subfloat[Layer $10$, Head $7$]{
    \includegraphics[width=0.25\linewidth]{figures/a10h7-1.pdf}
}
\caption{A significant number of the attention heads popular among the $70\%$ (heuristic) subnetworks attend to repeated tokens across the premise and context. Since the order of, \emph{e.g.}, ``doctor'' and ``president'' is reversed, the heads seem to identify either lexical overlap or constituent match, rather than subsequence match.}
\label{fig:attnmaps}
\end{figure*}
Instead of finding evidence for distinct, competing subnetworks, our results have suggested that the model ultimately generalizes by means of a dense collection of attention heads.
This suggests an alternative picture of generalization, which we refer to as the \ti{Heuristic Core Hypothesis}.
Specifically, we conjecture that the model can be seen as consisting of a ``heuristic core''---a subset of attention heads that are common to subnetworks at all sparsity levels.
The model generalizes by incorporating more attention heads, which can be seen as ``counter-heuristics''.
Different subsets of these heads improve generalization to different subcases.
In this section, we conduct further analysis to gain some understanding of how the heuristic core attention heads behave, and how they interact with the counter-heuristic heads.

\paragraph{How do the heuristic-core attention heads behave?}
Our analysis will be confined to MNLI/HANS for this section. 
\adithya{Remove the above statement if/when we add QQP analysis} 
We first look at the attention patterns exhibited by the heads popular among the heuristic ($70\%$) subnetworks.
Our expectation is that these attention heads extract simple, heuristic features---in particular, checking for lexical overlap between the two sentences.
Figure~\ref{fig:attnmaps} displays the attention maps for four such heads on one example taken from the \emph{subject-object swap} (lexical overlap) subcase of HANS.
The heads attend to words repeated across the premise and hypothesis. 
Table~\ref{tab:heurattn} quantifies this observation by means of a micro-average.
This pattern continues to hold when the relative ordering of words is swapped.
Therefore, the attention pattern hints at the head assimilating some lexical overlap feature.

\paragraph{How do the heuristic-core attention heads interact with the rest of the model?}
To investigate the nature of these heads further, we identify the heads occurring in all the heuristic subnetworks.
We then ablate them individually from the full model and observe how the in-domain and out-of-domain accuracies change, in Table~\ref{tab:ablations}.
None of the heads' ablation affects in-domain accuracy greatly.
For some (like $8.11$), their ablation leads to an increased accuracy on the OOD splits.
This implies that they contribute to heuristic behavior, as we would expect.

\begin{table}
    \centering
    \small
    \begin{tabular}{ccc}
    \toprule
    \textbf{Head} & \textbf{\makecell{Frequency, 70\%\\sparsity subnetworks}} & \textbf{\makecell{Attention between\\repeated words}}\\
    \midrule
    \makecell{Average\\all heads} & - & 4.3\%\\
    \midrule
    2.5 & 12/12 & 45.3\%\\
    3.7 & 12/12 & 54.9\%\\
    4.0 & 12/12 & 84.6\%\\
    8.11 & 12/12 & 58.0\%\\
    9.9 & 12/12 & 0.0\%\\
    10.10 & 12/12 & 2.5\%\\
    \bottomrule
    \end{tabular}
    \caption{The micro-average of the fraction of attention between repeated pairs of words across the premise/hypothesis, over the \emph{subject-object swap} subcase (lexical overlap) of HANS. The average is only taken over tokens that occur in both. We list the averaged fraction across all heads as a baseline.}
    \label{tab:heurattn}
\end{table}

Surprisingly, however, many heads seem to behave \emph{counter-heuristically} on ablation.
Moreover, the drops observed on ablating these heads is \emph{super-additive}.
As Figure~\ref{fig:3heads} shows, ablating the three counter-heuristic heads we identified leads to the OOD accuracy plummeting. 
Thus, these heads seem crucial to the generalization of the model.
As each appears in all of the heuristic subnetworks, they also seem to play an important role in heuristic behavior. 
This suggests that generalization involves a complex interaction between these heads in the heuristic core and the other attention heads.
A study of the non-heuristic components cannot be undertaken in isolation (reiterating the findings of~\citet{wen2023transformers}).

==> sections/competing_subnetwork_hypothesis.tex <==
We start by investigating three aspects of the Competing Subnetworks Hypothesis, observed by~\citet{taleoftwocircuits}.
\emph{First}, a rise in generalization is accompanied by a reduction in the model's \ti{effective size}, as the model switches from a dense, memorizing subnetwork to a sparse, generalizing one.
\emph{Second}, there exists a sparse generalizing subnetwork.
\emph{Third}, there exist two \emph{disjoint} subnetworks, one that generalizes and one that does not.

\begin{figure*}[t]
\centering
\subfloat[MNLI, $50\%$]{
    \includegraphics[width=0.335\linewidth]{figures/t50-kl-res-plot-trial.pdf}
}
\subfloat[MNLI, $70\%$]{
    \includegraphics[width=0.30\linewidth]{figures/t70-kl-res-plot-trial.pdf}
}
\subfloat[QQP, $30\%$]{
    \includegraphics[width=0.16\linewidth]{figures/eval-30-trial.pdf}
}
\subfloat[QQP, $60\%$]{
    \includegraphics[width=0.16\linewidth]{figures/eval-60-trial.pdf}
}
\caption{MNLI/HANS: At $50\%$ sparsity, the subnetworks operform within $3\%$ of the model on MNLI but show varying generalization. At $70\%$ sparsity, the subnetworks behave as pure heuristics despite respectable MNLI accuracy. The same trend also holds for QQP/PAWS, with sparsities of $30\%$ and $60\%$.  The solid line indicates full model performance. Figure~\ref{fig:multiprunefull} in Appendix~\ref{sec:fullresults} shows the corresponding plot for all subcases of HANS.}
\label{fig:multiprune}
\end{figure*}

\paragraph{Effective size \emph{increases} as the model generalizes}
First, we evaluate whether the rise in generalization is accompanied by a decrease in the \ti{effective size}, defined as the size of the smallest subnetwork that is \ti{faithful} to the model on a particular evaluation dataset $D$.
We say that a subnetwork is \ti{faithful} to a model on dataset $D$ if their accuracies are within $3\%$.
We report faithfulness using different choices of $D$---either the in-domain validation set, the out-of-domain validation sets, and the equally weighted combination of the two.
We prune each checkpoint to sparsities that are multiples of $5\%$.

The results are in Figure~\ref{fig:effsize}.
The effective size needed to approximate the model on the in-domain evaluation remains relatively flat over the course of training.
However, on both datasets, generalization is accompanied by an \ti{increase} in effective size.
These results suggest that, rather than switching from a dense, memorizing network to a sparse, generalizing one, the model generalizes by incorporating more components.

\begin{table*}
    \centering
    \small
    \begin{tabular}{cc|cccc}
        \toprule
        \multirow{2.5}{*}{\textbf{\makecell{Ablated Head}}} & \multicolumn{5}{c}{\textbf{Accuracy (\%)} 
 $\uparrow$}\\
        \cmidrule{2-6}
         & \textbf{\makecell{MNLI (matched)}} & 
\textbf{\makecell{SO-Swap [LO]}} & \textbf{\makecell{Prep [LO]}} & \textbf{\makecell{Embed-If [C]}} & 
\textbf{\makecell{Embed-Verb [C]}}\\
        \midrule
        None & 83.3 & 86.7 & 73.5 & 33.0 & 33.4\\
        \midrule
        \rowcolor{blue!30} 2.5 & 83.4$_{\uparrow 0.1}$ & 70.3$_{\downarrow 16.4}$ & 58.6$_{\downarrow 14.9}$ & 28.5$_{\downarrow 4.5}$ & 23.6$_{\downarrow 9.8}$\\
        \rowcolor{blue!30} 3.7 & 83.5$_{\uparrow 0.2}$ & 68.6$_{\downarrow 18.1}$ & 60.2$_{\downarrow 13.3}$ & 28.2$_{\downarrow 4.8}$ & 23.0$_{\downarrow 10.4}$\\
        \rowcolor{blue!30} 4.0 & 82.9$_{\downarrow 0.4}$ & 45.4$_{\downarrow 41.3}$ & 41.8$_{\downarrow 31.7}$ & 21.2$_{\downarrow 11.8}$ & 12.7$_{\downarrow 20.7}$\\
        \rowcolor{red!30} 8.11 & 81.0$_{\downarrow 2.3}$ & 88.3$_{\uparrow 1.6}$ & 76.5$_{\uparrow 3.0}$ & 37.6$_{\uparrow 4.6}$ & 34.1$_{\uparrow 0.7}$\\
        \rowcolor{red!30} 9.9 & 83.4$_{\uparrow 0.1}$ & 87.7$_{\uparrow 1.0}$ & 74.2$_{\uparrow 0.7}$ & 36.1$_{\uparrow 3.1}$ & 32.4$_{\downarrow 1.0}$\\
        10.10 & 81.5$_{\downarrow 1.8}$ & 84.7$_{\downarrow 2.0}$ & 72.2$_{\downarrow 1.3}$ & 41.1$_{\uparrow 8.1}$ & 38.7$_{\uparrow 5.36}$\\
        \bottomrule
    \end{tabular}
    \caption{The effects of ablating some heads occurring in all heuristic subnetworks from the full model. Surprisingly, many of these heads are implicated in \colorbox{blue!30}{counter-heuristic} behavior, as their ablation leads to reduced generalization. Ablating some leads to increased OOD accuracy, showing that they contribute more to \colorbox{red!30}{heuristic} behavior.}
    \label{tab:ablations}
\end{table*}

\paragraph{Sparser subnetworks generalize worse} 
In the previous section, we observed that the effective size needed to generalize increases over training.
In Figure~\ref{fig:perfvssparsity}, we plot the generalization accuracy of subnetworks pruned at higher sparsity levels.
We find that the generalization accuracy generally drops steadily at higher sparsity levels.
This constrasts with the algorithmic settings, such as the sparse parity task studied by~\citet{taleoftwocircuits}, where we might expect to see a phase transition when the sparsity drops below a threshold.

To investigate further, we prune the final model with $12$ different random seeds ($42$ through $53$) at two target sparsities -- $50\%$ (some generalization)  and $70\%$ (no generalization). 
All the subnetworks at 50\% sparsity perform similarly in domain -- within $3\%$ of the full model -- but their out-of-domain performance varies widely.
Moreover, different subnetworks generalize to different subcases.
Seed $49$ achieves $41.4\%$ at \emph{subject-object swap} (lexical overlap) but only $18.0\%$ at \textit{embedded under if} (constituent).
Seed $46$, on the other hand, achieves only $19.5\%$ at the former but $50.2\%$ at the latter.
Thus, pruning off different parts of the model seems to sacrifice generalization on different OOD subcases to varying degrees.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/ablated.pdf}
    \caption{Ablating just three of the attention heads (2.5, 3.7, and 4.0), occurring in all \emph{heuristic} subnetworks, severely degrades the model's generalization ability.}
    \label{fig:3heads}
\end{figure}

\paragraph{The heuristic subnetworks are subsets of generalizing subnetworks} As we prune more aggressively, \emph{all} of our subnetworks collapse to near-zero OOD accuracies, \emph{i.e.}, behave as pure heuristics (Figure~\ref{fig:multiprune}).
The ID accuracy remains at a respectable $74-76\%$, indicating that a large portion of model performance is explained by this relatively sparse heuristic subnetwork.
Contrary to what the Competing Subnetworks Hypothesis predicts, it is the heuristic subnetwork that is sparse.
Furthermore, it is a \emph{subset} of the partially generalizing subnetworks.
As Figures~\ref{fig:membership} and~\ref{fig:membership-qqp} in Appendix~\ref{sec:fullresults} show, the attention heads popular in the $70\%$ sparsity subnetworks are also among the most popular heads in the $50\%$ subnetworks.
The Spearman's Rho agreement coefficient between the frequencies of attention heads (among the $12$ pruned subnetworks) at $50\%$ and $70\%$ sparsity is $0.82$ for MNLI/HANS (very strong agreement) and $0.74$ for QQP/PAWS-QQP.

